Wiman and Arima theorems for quasiregular mappings

Generalizations of the theorems of Wiman and of Arima on entire functions are proved for spatial quasiregular mappings.

==> avv1_preprint.tex <==
% AVV.STY
% Kirjan "Inequalities for conformal invariants and quasiconformal mappings"
% tekemisess" tarvittavia virityksi"
% Eija Saario syksy 1993
% *************************************************************************

% Yht"l"t vasemmalle. Made by Joku Muu
% leqno.sty 14 Jun 85

%\def\@eqnnum{\hbox to .01pt{}\rlap{\rm \hskip -\displaywidth(\theequation)}}
%\def\@eqnnum{\hbox to .01pt{}\rlap{\normalshape \hskip -\displaywidth (\theequation)}}
\def\@eqnnum{\hbox to .01pt{}\rlap{\hskip -\displaywidth (\theequation)}}
% changed by P. S. 29.11.94 
% **************************************************************************

% Use "chapter" as "part" 

\def\part{\par \addvspace{4ex} \@afterindentfalse \secdef\@part\@spart} 
\def\@part[#1]#2{\ifnum \c@secnumdepth >\m@ne \refstepcounter{part}
\addcontentsline{toc}{part}{\thepart \hspace{1em}#1}\else
\addcontentsline{toc}{part}{#1}\fi { \parindent 0pt \raggedright 
 \ifnum \c@secnumdepth >\m@ne \large \bf Part \thepart \par\nobreak \fi \Large
\bf #2\markboth{}{}\par } \nobreak \vskip 3ex \@afterheading } 
\def\@spart#1{{\parindent 0pt \raggedright 
 \huge \bf 
 #1\par} \nobreak \vskip 3ex \@afterheading } 
\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus -1ex minus 
 -.2ex}{2.3ex plus .2ex}{\Large\bf}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-3.25ex plus -1ex minus 
 -.2ex}{1.5ex plus .2ex}{\large\bf}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-3.25ex plus
 -1ex minus -.2ex}{1.5ex plus .2ex}{\normalsize\bf}}
\def\paragraph{\@startsection
 {paragraph}{4}{\z@}{3.25ex plus 1ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsection
 {subparagraph}{4}{\parindent}{3.25ex plus 1ex minus 
 .2ex}{-1em}{\normalsize\bf}}

\def\l@part{\@dottedtocline{1}{0em}{0em}}
\def\l@section{\@dottedtocline{1}{1.5em}{2.3em}}
\def\l@subsection{\@dottedtocline{2}{3.8em}{3.2em}}
\def\l@subsubsection{\@dottedtocline{3}{7.0em}{4.1em}}
\def\l@paragraph{\@dottedtocline{4}{10em}{5em}}
\def\l@subparagraph{\@dottedtocline{5}{12em}{6em}}
% **************************************************************************

\def\thepart      {\Roman{part}}
\def\thesection      {\arabic{section}} % piste muutettu 13.9.94 P. S.
\def\thesubsection   {\thesection	.\arabic{subsection}}
\def\thesubsubsection{\thesubsection	.\arabic{subsubsection}}
\def\theparagraph    {\thesubsubsection .\arabic{paragraph}}
\def\thesubparagraph {\theparagraph     .\arabic{subparagraph}}
%\def\theequation     {$\thesection      .\arabic{equation}$}
\def\theequation     {\thesection      .\arabic{equation}} % 30.11.94
%\def\thefigure       {$\brm{\thesection .\arabic{figure}}$} % 5.12.94
\def\thefigure       {\thesection .\arabic{figure}}
%\def\thetable         {$\brm{\thesection .\arabic{table}}$}
\def\thetable        {\thesection  .\arabic{table}}
% ****************************************************************

\renewcommand{\fnum@figure}{{\bf Figure \thefigure}} % 14.9.94 P. S.
\renewcommand{\fnum@table}{{\bf Table \thetable}} %    & 5.12.94

%\def\figurename{${\brm Figure}$}% doesn't seem to work
%\def\tablename{${\brm Table}$}%

% ****************************************************************

% Definitions for new evironments
% ACHTUNG ! All environmnets use same counter 'own' and also the
% equations have same the same counter.  

\newcounter {own}
%\def\theown {$\brm{\thesection       .\arabic{own}}$} 
\def\theown {\thesection       .\arabic{own}} % 22.9.94 P. S.

% spaces between #.#. and Lemma (etc.) changed to fixed length 15.11.94  P. S.
% \bigskip's changed to \addvspace{\bigskipamount}'s 30.11.94

\newenvironment{lem}[1]{ 
\setcounter{own}{\value{equation}} \addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown.\ \, Lemma#1.} \sl}{\bigskip
\indent {\bf \theown.\hspace{1em}Lemma#1.} \sl}{\par\addvspace{\bigskipamount}
}

\newenvironment{thm}[1]{
\setcounter{own}{\value{equation}} \addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown.\ \, Theorem#1.} \sl }{\bigskip
\indent {\bf \theown.\hspace{1em}Theorem#1.} \sl }{\par\addvspace{\bigskipamount}
}

\newenvironment{nonsec}{\bf 
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount} 
%\indent \theown.$\ \,$}{$\!$.\ \ \ }
\indent \theown.\hspace{1em}\ignorespaces }{\unskip .\ \ \ }


\newenvironment{subsec}[1]{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
\indent {\bf \theown.\hspace{1em}#1\unskip$\, \ $} }{}


\newenvironment{pf}{
%\medskip
\par\addvspace{-\smallskipamount}
\indent {\bf Proof.}$\,\ $}{
\par\addvspace{\bigskipamount}
}

\newenvironment{cor}{
\setcounter{own}{\value{equation}} \addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. \ \ Corollary.\,\ }  \sl }{\bigskip
\indent {\bf \theown.\hspace{1em}Corollary.\,\ }  \sl }{\par\addvspace{\bigskipamount}
}


\newenvironment{conj}{
\setcounter{own}{\value{equation}} \addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. \ \ Conjecture.\,\ }  \sl }{\bigskip
\indent {\bf \theown.\hspace{1em}Conjecture.\,\ }  \sl }{\par\addvspace{\bigskipamount}
}




\newenvironment{prop}{
\setcounter{own}{\value{equation}} \addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. \ \ Proposition.\,\ }  \sl }{\bigskip
\indent {\bf \theown.\hspace{1em}Proposition.\,\ }  \sl }{\par\addvspace{\bigskipamount}
}


 
\newenvironment{exerc}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $Exercises.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Exercises.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{exercise}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $Exercise.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Exercise.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{diagrams}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $Diagrams.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Diagrams.$\, \ $} }{\par\addvspace{\bigskipamount}
}


\newenvironment{exmp}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown.$\ \ $ Example.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Example.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{examples}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $ Examples.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Examples.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{defin}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $ Definition.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Definition.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{rem}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $ Remark.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Remark.$\, \ $} }{\par\addvspace{\bigskipamount}
}


\newenvironment{remarks}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $Remarks.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Remarks.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{notes}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $ Notes.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Notes.$\, \ $} }{\par\addvspace{\bigskipamount}
}

\newenvironment{notation}{
\setcounter{own}{\value{equation}}\addtocounter{equation}{1}
\refstepcounter{own}
\par\addvspace{\bigskipamount}
%\indent {\bf \theown. $\ \ $ Notation.$\, \ $} }{\bigskip
\indent {\bf \theown.\hspace{1em}Notation.$\, \ $} }{\par\addvspace{\bigskipamount}
}

% **************************************************************
% Definitions for new list environments.

\newcounter{lista1}
\newcounter{lista2}
\newcounter{lista3}
\newcounter{lista4}

\newenvironment {nlist}
{\begin{list} {$(\arabic{lista1})$}
{\usecounter{lista1} \setcounter{lista1}{0}}}{\end{list}}

\newenvironment {nlist2}
{\begin {list}{$(\arabic{lista2})$}{\usecounter{lista2} 
\setcounter{lista2}{1} \parskip 0pt \partopsep 0pt}}{\end{list}}


\newenvironment {abclist}
{\begin {list}{(\alph{lista3})}{\usecounter{lista3}}}{\end{list}}

\newenvironment {abclist2}
{\begin {list}{(\alph{lista4})}{\usecounter{lista4} \setcounter{lista4}{1} 
\parskip 0pt \partopsep 0pt }}{\end{list}}

\newenvironment{lb}
{\parindent 1.1cm}{}

% Next trick is not so clever way to handle first list item in the
% case, where the list should begin from the same line as the text
% before the item. Example:  

% 2.1 Remark (1) ....
%    \item 
%    \item 

%\def\hang{\hangindent 1.1cm\parindent \hangindent}  changed 10.11.94 and 5.12.94 by P. S.
\def\hang{\hangindent\leftmargini}
\def\fitem{\hang}
\def\ftext{\medskip

\hang\textindent}

% fitemlist environment added by P. S. 10 Nov 94 
% The previous definition doesn't work when \fitem has a sublist
% To produce

% 2.1 Remark. (1) ...
%      (a) ...
%      (b) ...
% (2) ... 
% (3) ...

% type

% ... \fitem{(1)} ... 
%  \begin{fitemlist}
%   \item[(a)] ...
%   \item[(b)] ...
%  \end{fitemlist}
% \begin{nlist2}
%  \item ...
% \end{nlist2}

\newenvironment{fitemlist}
{\begin{list}{}{\advance\leftmargin\leftmarginii}}{\end{list}}

% *******************************************************************



%\input mssymb
\input m.tex
\setlength{\textwidth}{150truemm} \setlength{\textheight}{235truemm}
\addtolength{\topmargin}{-15mm}
\setlength{\oddsidemargin}{6mm}
\setlength{\evensidemargin}{6mm}
\parskip 0pt plus 2pt

\parindent\leftmargini % same as item indent



% tex-maarittelyt

%\magnification=\magstep1

%\hsize=15truecm

%\vsize=23.5truecm

\def\ts{\textstyle}

%\font\ff=eusm10     % KAUNIIN K:n MAARITTELY

%\def\th{\mathop{\rm th}\nolimits}

\def\thx{\mathop{\rm thx}\nolimits}

\def\thy{\mathop{\rm thy}\nolimits}

\def\thr{\mathop{\rm thr}\nolimits}

%\def\arth{\mathop{\rm arth}\nolimits}

%\newdimen\refskip

%\refskip=20pt                                                        %

%\def\ref #1 #2\par{\par\noindent\rlap{#1}\hskip\refskip

%\hangindent\refskip #2}

%\def\kohta #1 #2\par{\par\noindent\rlap{#1}\hskip\refskip

%\hangindent\refskip #2\par}



\def\A{{\cal A}}

\def\B{{\cal B}}  % m.tex:in \B ei ole kaytossa enaan

%\def\K{\hbox{\ff K}}

%\def\E{\hbox{\ff E}}

\def\F{{\cal F}}

\def\J{{\cal J}}

\def\M{{\cal M}}

\def\N{{\cal N}}

\def\O{{\cal O}}

\def\U{{\cal U}}

\def\WT{{\cal W}{\cal T}}

\def\X{{\cal X}}

\def\Y{{\cal Y}}



\def\1{{\hbox{\rm 1}\hskip-0.38em\hbox{\rm 1}}}



%\def\C{\Bbb C} oli 10pt tekstia, tehdaan uusi:

%\font\bbb=msym10 scaled 1200
\def\C{\mbox{\bbb C}}

\def\isowedge{{\textstyle\bigwedge\limits}}

%\def\1{\mbox{$\Bbb 1$}}

\def\Re{{\,\rm Re}}

\def\Im{{\,\rm Im}}

\def\osc{{\rm osc}}

\def\inter{{\rm int}}

\def\supp{{\rm supp}\,}

\def\loc{{\rm loc}}

\def\dist{{\rm dist}\,}

\def\diver{{\rm div}\,}

\def\epsilon{\varepsilon}



%\footline={\ifnum\pageno=1 \ffolio

%\else \hfill\rm\folio\hfill\fi}

%\headline={\ifnum\pageno=1 \ffolio

%\else \hfill\rm V\"ais\"al\"a\hfill\fi}

%\def\ffolio{\hfil\null}

%\overfullrule=0pt

%\def\sqr#1#2{{\vcenter{\hrule height.#2pt

%      \hbox{\vrule width.#2pt height#1pt \kern#1pt

%         \vrule width.#2pt}

%       \hrule height.#2pt}}}

%\def\op{\mathchoice\sqr34\sqr34\sqr{2.1}3\sqr{1.5}3}

%\def\beop{\mathchoice\sqr56\sqr56\sqr{2.1}5\sqr{1.5}5}

%\def\Jbeop{$\op $}

%\def\eop{\ifmmode\op\else\Jbeop\fi }



%%%%%%%%%%%%%%%%

%\pagestyle{myheadings}
%\markboth{\today}{\today}


%\newcommand{\vse}{\vspace{.2in}}

%\newcommand{\np}{\newpage}




